Verde: Verification via Refereed Delegation for Machine Learning Programs

Machine learning programs, such as those performing inference, fine-tuning, and training of LLMs, are commonly delegated to untrusted compute providers. To provide correctness guarantees for the client, we propose adapting the cryptographic notion of refereed delegation to the machine learning setting. This approach enables a computationally limited client to delegate a program to multiple untrusted compute providers, with a guarantee of obtaining the correct result if at least one of them is honest. Refereed delegation of ML programs poses two technical hurdles: (1) an arbitration protocol to resolve disputes when compute providers disagree on the output, and (2) the ability to bitwise reproduce ML programs across different hardware setups, For (1), we design Verde, a dispute arbitration protocol that efficiently handles the large scale and graph-based computational model of modern ML programs. For (2), we build RepOps (Reproducible Operators), a library that eliminates hardware "non-determinism" by controlling the order of floating point operations performed on all hardware. Our implementation shows that refereed delegation achieves both strong guarantees for clients and practical overheads for compute providers.

==> Makefile <==
# LaTeX Makefile
#
# Author: Jay Bosamiya <jaybosamiya AT gmail DOT com>
#
# Always find the latest version at
#    https://github.com/jaybosamiya/latex-paper-template/
#
# Alternatively, run `make update-makefile` to pull the latest
# version.

#   ____             __ _                       _   _
#  / ___|___  _ __  / _(_) __ _ _   _ _ __ __ _| |_(_) ___  _ __
# | |   / _ \| '_ \| |_| |/ _` | | | | '__/ _` | __| |/ _ \| '_ \
# | |__| (_) | | | |  _| | (_| | |_| | | | (_| | |_| | (_) | | | |
#  \____\___/|_| |_|_| |_|\__, |\__,_|_|  \__,_|\__|_|\___/|_| |_|
#                         |___/

# If set to 't', all .tex files in the current directory should be
# compiled over to .pdf files.
ALL_FILES_MODE?=

# If set then MAIN_TARGET is used as the root tex file of the project
# to be built.
MAIN_TARGET?=

################## DON'T CHANGE ANYTHING BEYOND THIS LINE ####################

#     _         _                        _   _        ____        _
#    / \  _   _| |_ ___  _ __ ___   __ _| |_(_) ___  |  _ \ _   _| | ___  ___
#   / _ \| | | | __/ _ \| '_ ` _ \ / _` | __| |/ __| | |_) | | | | |/ _ \/ __|
#  / ___ \ |_| | || (_) | | | | | | (_| | |_| | (__  |  _ <| |_| | |  __/\__ \
# /_/   \_\__,_|\__\___/|_| |_| |_|\__,_|\__|_|\___| |_| \_\\__,_|_|\___||___/
#

.PHONY: all
TEXFILES:=$(wildcard *.tex)

AUTOPICK:=main.tex

ifeq ($(ALL_FILES_MODE), t)
ifneq ($(MAIN_TARGET),)
all:
	@echo "Both ALL_FILES_MODE and MAIN_TARGET are set."
	@echo ""
	@echo "Do you mean to compile all of them individually to PDFs?"
	@echo "  If so, please change over to ALL_FILES_MODE"
	@echo ""
	@echo "Do you mean to compile it to a single PDF?"
	@echo "  If so, please set MAIN_TARGET"
	@echo ""
	@echo "Quitting."
else
all: $(TEXFILES:.tex=.pdf)
endif
# End of ALL_FILES_MODE
else ifneq ($(MAIN_TARGET),)
all: $(MAIN_TARGET:.tex=).pdf
# End of MAIN_TARGET
else
all:
ifeq ($(words $(TEXFILES)), 1)
all: $(TEXFILES:.tex=.pdf)
else ifeq ($(words $(filter $(AUTOPICK),$(TEXFILES))), 0)
all:
	@echo "Found $(words $(TEXFILES)) .tex files."
	@echo ""
ifeq ($(words $(TEXFILES)), 0)
else
	@echo "Do you mean to compile all of them individually to PDFs?"
	@echo "  If so, please change over to ALL_FILES_MODE"
	@echo ""
	@echo "Do you mean to compile it to a single PDF?"
	@echo "  If so, please set MAIN_TARGET"
	@echo ""
endif
	@echo "Quitting."
else
AUTOROOTCHOICE:=$(firstword $(foreach V,$(AUTOPICK),$(filter $(V),$(TEXFILES))))
all: $(warning Found multiple .tex files. Automatically chosing likely root as $(AUTOROOTCHOICE). Set either MAIN_TARGET or ALL_FILES_MODE to squash this warning.) $(AUTOROOTCHOICE:.tex=.pdf)
endif
endif

LATEXRUN:=python3 ./.latexrun -O .latex.out
# Note: We use latexrun from a slightly more up-to-date fork available
# at https://github.com/Nadrieril/latexrun
# The original can be found at https://github.com/aclements/latexrun

.PHONY: FORCE
%.pdf: FORCE ./.latexrun
	@$(LATEXRUN) $*.tex

.PHONY: clean
clean: ./.latexrun
	@$(LATEXRUN) --clean-all
	@echo "Finished cleaning up"

./.latexrun:
	@echo "Unable to find .latexrun in the current directory."
	@echo "Downloading it!"
	@wget https://raw.githubusercontent.com/Nadrieril/latexrun/master/latexrun -O $@

.PHONY: update-makefile
update-makefile:
	@echo "Updating the current Makefile in-place"
	@wget --quiet --unlink https://raw.githubusercontent.com/jaybosamiya/latex-paper-template/master/Makefile -O Makefile


==> protocols/bisection_tree.tex <==
\begin{algorithm}
\begin{algorithmic}
\STATE {\bf Participants}: Players $P_0, P_1$
\STATE {\bf Input}: Merkle tree roots $\rt_0, \rt_1$
\STATE
\STATE $(\currt_0, \currt_1) := (\rt_0, \rt_1)$
\STATE $(\start, \sfend) = (0, n)$
\FOR{$i = 0$ to $\log n$}
    \STATE $P_1, P_2$ send $(l_1, r_1), (l_2, r_2)$, respectively.
    \STATE If $H(l_i, r_i) \neq \currt_i$ for either $i$, then $R$ eliminates $P_i$
    \IF{$l_1 = l_2$}
        \STATE $(\currt_0, \currt_1) = (r_0, r_1)$
        \STATE $\start = (\start+\sfend)/2$
    \ELSE{}
        \STATE $(\currt_0, \currt_1) = (l_0, l_1)$
        \STATE $\sfend = (\start+\sfend)/2$
    \ENDIF
\ENDFOR
\STATE Let $\displeaves = (\currt_0, \currt_1)$ 
\STATE Disputed index $\dispidx = \start$
\STATE Referee outputs: $(\dispidx, \displeaves)$
\STATE
\end{algorithmic}
\caption{{\bf Dispute bisection game.} The players and the referee 
identify the first step the two players diverged in their computation.}
\label{alg:protocol_bisection_background}
\end{algorithm}


